Rethinking Misalignment to Raise the Bar for Heap Pointer Corruption

Heap layout randomization renders a good portion of heap vulnerabilities unexploitable. However, some remnants of the vulnerabilities are still exploitable even under the randomized layout. According to our analysis, such heap exploits often abuse pointer-width allocation granularity to spray crafted pointers. To address this problem, we explore the efficacy of byte-granularity (the most fine-grained) heap randomization. Heap randomization, in general, has been a well-trodden area; however, the efficacy of byte-granularity randomization has never been fully explored as \emph{misalignment} raises various concerns. This paper unravels the pros and cons of byte-granularity heap randomization by conducting comprehensive analysis in three folds: (i) security effectiveness, (ii) performance impact, and (iii) compatibility analysis to measure deployment cost. Security discussion based on 20 CVE case studies suggests that byte-granularity heap randomization raises the bar against heap exploits more than we initially expected; as pointer spraying approach is becoming prevalent in modern heap exploits. Afterward, to demystify the skeptical concerns regarding misalignment, we conduct cycle-level microbenchmarks and report that the performance cost is highly concentrated to edge cases depending on L1-cache line. Based on such observations, we design and implement an allocator suited to optimize the performance cost of byte-granularity heap randomization; then evaluate the performance with the memory-intensive benchmark (SPEC2006). Finally, we discuss compatibility issues using Coreutils, Nginx, and ChakraCore.

==> fig/sunspider.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
Application        & Task           & w/o RUMA     & w/  RUMA     & Average Performance Penalty \\ \hline \hline
Safari Web Browser & SunSpider benchmark  & 129.74 msec  & 130.02 msec  & 0.22\% \\ \hline
Adobe Flash Player & Quicksort algorithm implementation  & 7348.4 msec  & 7381.0 msec  & 0.44\% \\ \hline
Adboe Acrobat Pro  & PDF file rendering         & 15883.6 msec & 15902.2 msec & 0.12\% \\ \hline
\end{tabular}

